Distinguishing Between Roles of Football Players in Play-by-play Match Event Data

Over the last few decades, the player recruitment process in professional football has evolved into a multi-billion industry and has thus become of vital importance. To gain insights into the general level of their candidate reinforcements, many professional football clubs have access to extensive video footage and advanced statistics. However, the question whether a given player would fit the team's playing style often still remains unanswered. In this paper, we aim to bridge that gap by proposing a set of 21 player roles and introducing a method for automatically identifying the most applicable roles for each player from play-by-play event data collected during matches.

==> tex/considerations.tex <==
\section{Early experiments}
\label{sec:considerations}

\change{Our first approach in extracting player roles from event data has been to regard this as being an unsupervised learning task. One advantage of this approach was that the data would ideally point out the number of roles available, which could be provided with a label later on. To add domain knowledge to the model we asked a large group of experts to define 'is-similar' and 'is-different' constraints for a large set of players. From these constraint based clustering experiments we learned that it is almost impossible to detect clear cluster bounds. One of the main issues in this is the rather continues mapping of players, e.g. players 1 and 2 are similar, players 2 and 3 are similar but players 1 and 3 are different. Therefore we now approach this as being a supervised learning task, where expert knowledge is used in determining the labels for players.}
